Sketching for low-rank nonnegative matrix approximation: Numerical study

We propose new approximate alternating projection methods, based on randomized sketching, for the low-rank nonnegative matrix approximation problem: find a low-rank approximation of a nonnegative matrix that is nonnegative, but whose factors can be arbitrary. We calculate the computational complexities of the proposed methods and evaluate their performance in numerical experiments. The comparison with the known deterministic alternating projection methods shows that the randomized approaches are faster and exhibit similar convergence properties.

==> parts/problem_statement.tex <==
\section{Problem statement}

However, small negative numbers arise in the approximations as aftifacts of the approximation. In case of Smoluchowski equations the solution $n(v_1, v_2, t)$ cannot contain negative entries. Thus, after the numerical investigation of the initial problem it is natural to provide some post-processing procedures allowing to obtain a rank-r nonnegative approximation of the initial matrix elementwise. In recent work \cite{song2020nonnegative} a simple iterative approach based on alternating projections (see algortithm \ref{alg:LRNMF_org}. Each iteration by the method of alternating projections costs $O(N^3)$ operations for $N \time N$ matrix. The main aim of this work is decrease of this complexity with possible construction of an algorithm allowing to perform processing of only factors of the low-rank approximation without straight-forward work with full matrix.

Idea from algorithms \ref{alg:LRNMF_rsvd_it} is very natural and allows to decrease the complexity from $O(N^3)$ to $O(N^2 r)$ operations by replacing of the SVD by randomized-SVD operation. This ideas allow to keep robustness of the updated algorithm with significantly faster construction of the result. However, the second projection to the manifold of nonnegative matrices still requires processing of all elements of the constructed approximation.

Our further idea is additional randomization of the approximations vie the adaptive cross approximation method which requires only $O(N r^2)$ evaluations of the entries of the target matrix $A_{ij}$ or grid function $A(i,j)$. If one can compute the any element without storage of the whole matrix then adaptive cross approximation allows to compress extremely huge amounts of data in really modest times. Thus, we replace a projector on the manifold of rank-r matrices by call of the adaptive cross approximation with additional condition on evaluation of the matrix elements :
$$\text{CROSS}( \max\left(A^{(r)}_{i,j}, 0 \right) ).$$
Such a trick allows us to avoid a straightforward projection of the approximation on the manifold of the nonnegative matrices but breaks the standard convergence criteria and the robustness of methodology. Nevertheless, our practice shows that it works and allows to filter number of negative entries by 10-100 times after just 5-10 iterations. Maybe this trick can be considered as a sort of fast filtering which can be done after each time-integration step instead of the long post-processing procedures. 

We present a brief analysis of properties of the considered methodology in table \ref{tab:algorithms}. The basic LRNMF method is robust but can be easily accelerated via changing of SVD-based projection to low-rank manifold by randomized SVD. This modification allows to accelerate the procedure significantly without visible difference in terms of convergence \ref{fig:convergence} or quality of the final accceleration. 

However, additional decrease of complexity and memory requirements can be done via the nonnegative cross approximation technique but this trick provokes a significant loss in accuracy and robustness. Moreover, the stopping criteria for the convergence of the iterative process has to be something new because we seek to avoid the exploitation of all elements of the initial matrix.

\begin{figure}
\includegraphics[width=0.28\textwidth]{1024_t25_r8_h1e-1svd_neg_part.png}~
\includegraphics[width=0.28\textwidth]{1024_t25_r15_h1e-1svd_neg_part.png}~
\includegraphics[width=0.28\textwidth]{1024_t25_r20_h1e-1svd_neg_part.png}~
\includegraphics[width=0.28\textwidth]{1024_t25_r25_h_1e-1svd_neg_part.png}~
\caption{\label{fig:NegPart}Negative elements of the approximations $A_r$ of rank $r$ of the analytical solution at the $t = 25$ with grid step $h = 0.1$ and $N = 1024$ nodes per axis. One may see that after a good approximation by SVD the compressed solutions contain many small negative elements. }
\end{figure}

\begin{table}[ht!]
    \centering
    \begin{tabular}{|c|c|c|c|c|}
        \hline
          N  & r &$||A - A_r||_F$ & \# negative elements & $\min$ el. in $A_r$ \\
          \hline
         256 &  8 &  $6.87 \cdot 10^{-3}$ &  2276 &  $9.378 \cdot 10^{-5}$\\
         256 & 10 &  $1.8 \cdot 10^{-4}$ &  1020 &  $2.0975 \cdot 10^{-7}$ \\
         256 & 15 & $4.18 \cdot 10^{-8}$ &  45 &  $6.57 \cdot 10^{-10}$ \\
         256 &  20 &  $7.96 \cdot 10^{-13}$ &  1 &  $7.5683 \cdot 10^{-17}$\\
         \hline
         512 &  8 &  $6.34 \cdot 10^{-2}$ & 43130 &  $3.8 \cdot 10^{-4}$ \\
         512 &  15 &  $1.17 \cdot 10^{-4}$ &  15190 &  $3.9541 \cdot 10^{-7}$ \\
         512 &  20 &  $9.377 \cdot 10^{-8}$ &  8069 &  $9.2254 \cdot 10^{-10}$ \\
         512 &  25 &  $7.96\cdot10^{-12}$ &  2010 &  $1.149 \cdot 10^{-13}$ \\
         \hline
         1024 &  8 &  0.182 &  278862 &  $8.86 \cdot 10^{-3}$ \\
         1024 & 15 & $4.289 \cdot 10^{-3}$ & 215100 & $1.616 \cdot 10^{-5} $ \\
         1024 & 20 & $1.12 \cdot 10^{-4}$  & 165531 & $3.8976 \cdot 10^{-7}$ \\
         1024 & 25 & $4.395 \cdot 10^{-7}$ & 112344 & $1.3827 \cdot 10^{-9}$ \\
         \hline
    \end{tabular}
    \caption{Approximation error in $|| \cdot ||_F$ of the analytical solution with at $T = 25$ and fixed grid step $h = 0.1$ with use of $N$ grid nodes per each axis}
    \label{tab:neg_elements}
\end{table}


\begin{algorithm}[h!]
\caption{LRNMF basic algorithm}\label{alg:LRNMF_it}
\begin{algorithmic}[1]
\Procedure{LRNMF iteration}{$A^{(r)}$}
\State Fill the matrix $A^{(+)}_{i,j} = \max\left( A^{(r)}_{i,j}, 0 \right) $  \\
\Comment costs $O(N^2)$ operations, projection to manifold of nonnegative matrices
\State Compute $A^{(r)}_{new} = U_r \Sigma_r V_r$  \\
\Comment result of rank-r truncated SVD of $A^{(+)}$, costs $O(N^3)$ operations, optimal projection to manifold of rank-r matrices
\State Return $A^{(r)}_{new}$, $||A^{(r)}_{new} - A^{(r)}||_F$ \\
\Comment costs $O(N^2)$ operations
\Procedure{Updates}{$A_{k}$, approximation from previous iteration }
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h!]
\caption{modified LRNMF algorithm}\label{alg:LRNMF_rsvd_it}
\begin{algorithmic}[1]
\Procedure{LRNMF iteration}{$A^{(r)}$}
\State Fill the matrix $A^{(+)}_{i,j} = \max\left( A^{(r)}_{i,j}, 0 \right) $ \\
\Comment costs $O(N^2)$ operations, projection to manifold of nonnegative matrices
\State Compute $A^{(r)}_{new} = \tilde{U}_r \tilde{\Sigma}_r \tilde{V}_r$ \\
\Comment result of rank-r randomized SVD of $A^{(+)}$, practically costs $O(N^2 \cdot r)$ operations, quasi-optimal projection to manifold of rank-r matrices
\State Return $A^{(r)}_{new}$, $||A^{(r)}_{new} - A^{(r)}||_F$  \\
\Comment costs $O(N^2)$ operations
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[h!]
\caption{Nonnegative adaptive cross sampling}\label{alg:LRNMF_cross_it}
\begin{algorithmic}[1]
\Procedure{LRNMF iteration}{$A^{(r)} = U^{(r)} V^{(r)}$}
\State Compute  $U^{(r)}_{new} V^{(r)}_{new} = \text{CROSS}( \max\left(A^{(r)}_{i,j}, 0 \right) )$ \\
\Comment $A^{(r)_{i,j}$ can be evaluated on-the-fly via scalar product of $i$-th row of matrix $U^{(r)}$ by $j$-th column of matrix $V^{(r)}$. \\
CROSS procedure returns automatically the factors $U^{(r)}_{new}$, $V^{(r)}_{new}$ corresponding to the update of the skeleton decomposition of the target matrix $A$.  \\
The complexity of this step is $O(N r^2)$ evaluations of target function $\max\left(A^{(r)_{i,j}, 0 \right)$ having the cost $O(r)$ operations. Thus, total complexity is $O(N r^3)$.
\State Return $U^{(r)}_{new}$, $V^{(r)}_{new}$, $||U^{(r)}_{new} - U^{(r)}||_F + ||V^{(r)}_{new} - V^{(r)}||_F$  \\
\Comment costs $O(N r)$ operations
\end{algorithmic}
\end{algorithm}

\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
         Algorithm & Complexity of iteration & Robustness & Storage \\
         \hline
         LRNMF & $O(N^3)$ & + & $O(N^2)$ \\
         LRNMF with R-SVD & $O(N^2 r)$ & + & $O(N^2)$ \\
        Nonnegative Adaptive Cross & $O(N r^3)$ & -- & $O(N r)$  \\
        \hline
    \end{tabular}
    \caption{Properties of the studied algorithms. Complexity, robustness, memory requirements. }
    \label{tab:algorithms}
\end{table}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{512_512_t25_r12_h1e-1_sigmas_manual_correction.png}
    \includegraphics[scale=0.5]{512_512_t25_r12_h1e-1_sigmas_manual_correction_zoom.png}
    \caption{Left panel: decrease of singular values $\sigma_i$, $i>12$ when the approximation of rank $r=12$ is applied within the iterations of algorithm \ref{alg:LRNMF_it}.  Right panel: almost ideal approximation of the first $r=12$ singular values during the LRNMF iterations during the decrease of other singular values. }
    \label{fig:sigmas_decrease}
\end{figure}

\begin{figure}
    \centering
    \includegraphics{convergrence_LRNMF_rsvd.png}
    \caption{Convergence of the approximations constructed by Algorithms  \ref{alg:LRNMF_it} and \ref{alg:LRNMF_rsvd_it}. One may see the very same results but cost of each iteration by \ref{alg:LRNMF_rsvd_it} is significantly lower. LRNMF requires 202.42 seconds and modification of LRNMF with randomize SVD takes only 142.57 seconds.}
    \label{fig:convergence}
\end{figure}
